Understanding Rulelog Computations in Silk

Rulelog is a knowledge representation and reasoning language based on logic programming under the well-founded semantics. It is an extension of the language of Flora-2 and so supports inheritance and other object-oriented features, as well as the higher-order syntax of Hilog. However, Rulelog rules may also contain quantifiers and may be contra-positional. In addition, these rules are evaluated in the presence of defeasibility mechanisms that include rule cancellation, rule priorities, and other aspects. Rulelog programs are sometimes developed by loosely coordinated teams of knowledge engineers (KEs) who are not necessarily programmers. This requires not only declarative debugging support, but also support for profiling to help KEs understand the overall structure of a computation, including its termination properties. The design of debugging and profiling tools is made more challenging because Rulelog programs undergo a series of transformations into normal programs, so that there is a cognitive distance between how rules are specified and how they are executed. In this paper, we describe the debugging and profiling environment for Rulelog implemented in the integrated development environment of the Silk system. Our approach includes an interface to justification graphs, which treat why-not and defeasibility as well as provenance of the rules supporting answers. It also includes tools for trace-based analysis of computations to permit understanding of erroneous non-termination and of general performance issues. For semantically correct cases of the non-terminating behavior, Silk offers a different approach, which addresses the problem in a formally sound manner by leveraging a form of bounded rationality called restraint.

==> overall-process.tex <==
\section{Overall Process of Knowledge Debugging} 

The tools we have described can be combined in a number of ways.
The typical process of knowledge debugging goes as follows.  
A user runs a (test) query of interest.  
If the execution of the query does not take an
unexpectedly/undesirably large amount of time or space, there is no
performance/termination issue.  The user looks at the answers to the query,
and employs the justification tools to examine the explanation of those answers
in terms of supporting conclusions and their associated assertions (rules
knowledge).
Along the way, the user looks for wrong or missing conclusions,
and wrong or missing rules.  The user may issue some other related queries 
as part of this investigation, and look at their explanations as well.  

However, if execution of the query does take an unexpectedly/undesirably 
large amount of time or space, there is a performance/termination issue.  
At this point, the user needs to determine whether the runaway is due to
non-termination or merely due to an inefficient computation. The first step
in determining the culprit is to look at the table dump of the trace.
If these show very large terms with deeply nested repeated function symbols,
non-termination is the likely problem, and Terminyzer can be further
employed to find the actual rule sequences that cause the problem.
Otherwise,
the user would use the table dump and the forest log tools to identify foci
of computational effort, by looking for  
large tables (via table dump) or large recursive components (via forest
log).
The user next drills down 
progressively from the macroscopic (more aggregated and general) 
to the microscopic (more detailed and specific).  
Once sufficiently microscopic, the user then also employs the 
justification tools (as described above)---and/or employs 
restraint, especially in order to ensure termination (e.g., by limiting
term size).  

As usual in any kind of debugging, the above steps are iterated as needed.     





==> restraint.tex <==
\section{Restraint: Bounded Rationality and Prevention of Runaway}
\label{sec-restraint}

% future version:
% give more details, esp. examples

%Another advanced way to control runaways is to use \emph{restraint},
%an approach to bounded rationality (and pragmatic incompleteness) that
%is semantically sound despite non-monotonicity \cite{GroS13}.  With
%restraint, the semantics of inferencing---and thus corresponding
%computation---is limited in well-defined way; answers derived after
%the limits have been reached are given the truth value of
%\emph{undefined}.

While Terminyzer is used for finding \emph{mistakes} in user's
knowledge base, 
%i.e., in situations when runaway computation is not intended, 
restraint may be used when the knowledge base is \emph{correct}, but has an infinite model.

%a. This typically occurs when the user query of interest or one of its
%subqueries has an infinite number of answers, but only the first few
%need to be returned to the user.

% future version:  say the u means ``do not bother'', and gen'lize WFS
%One type of restraint is to limit a norm on subgoals, e.g., term size or
%depth, to be upper-bounded by a constant, 
%which is called the \emph{radius}.
%By setting the radius to a small enough value, 
%radial restraint can be used to prevent runaways altogether. 
% future version: talk about setting the norm too 

% future version:  show the numberline example

Section~\ref{subsec:restraint} discussed how radial restraint can be
used for non-termination, but there are several other useful types of
restraint as well.  In \emph{skipping} restraint, conditions are
specified (via rules) for when some other rules instances should be
skipped, i.e., treated as having undefined truth value.  In
\emph{unsafety} restraint: a literal that is (irremediably)
% future version:  irremediably here means wrt subgoal reordering delay
unsafe with respect to NAF is treated
as having undefined truth value. Likewise, an
external-query (a.k.a. \emph{sensor}) literal that is
unsafe with respect to binding mode requirements 
% of the external query/predicate
is treated as having undefined truth value.  
% future version:  use the naf-unsafety.silk example
In \emph{unreturn} restraint, an external-query literal that 
does not return---e.g., due to network failure or server failure ---
is treated as having undefined truth value.
In some situations,
unsafety and unreturn restraints are preferable to
throwing an error.
% future version:  elaborate that they avoid ``barfing''
% future version:  paragraph break here
Radial and skipping restraint are \emph{voluntary} kinds of bounded 
rationality:  the user specifies desired limits on reasoning 
via meta-rules knowledge.
The limitation is cleanly semantic and specified as part of the knowledge
base itself.  
By contrast, unsafety and unreturn are \emph{involuntary}:  
limitations on reasoning are imposed by the circumstances of the 
inferencing mechanism and/or external environment.  

All the above types of restraint straightforwardly combine
with each other.  They furthermore straightforwardly combine
with the ``anytime'' approach
to temporally bounded rationality \cite{DeBo88,RuWe91a}.
In \emph{anytime} restraint, a series of increasingly complete
inferencing-result sets are computed and when a time limit
is reached, the best one computed so far is
returned.  For instance a restraint radius is progressively incremented until
the time limit is reached.  

% future version:  elaborate how restraint is baked in to the K / semantics
% and inferencing mechanism, and presented via answers and 
% justification/explanation

%%%%

% future version:  (maybe in different paper)
% undefined traversal 
% use call dep graph fm increm tabling, as way to understand dep in SCC's,
% wo/ having to use forestlog

%%%%

